DATCloud: A Model-Driven Framework for Multi-Layered Data-Intensive Architectures

The complexity of multi-layered, data-intensive systems demands frameworks that ensure flexibility, scalability, and efficiency. DATCloud is a model-driven framework designed to facilitate the modeling, validation, and refinement of multi-layered architectures, addressing scalability, modularity, and real-world requirements. By adhering to ISO/IEC/IEEE 42010 standards, DATCloud leverages structural and behavioral meta-models and graphical domain-specific languages (DSLs) to enhance reusability and stakeholder communication. Initial validation through the VASARI system at the Uffizi Gallery demonstrates a 40% reduction in modeling time and a 32% improvement in flexibility compared to manual methods. While effective, DATCloud is a work in progress, with plans to integrate advanced code generation, simulation tools, and domain-specific extensions to further enhance its capabilities for applications in healthcare, smart cities, and other data-intensive domains.

==> Xevaluation.tex <==
\section{CASE STUDY AND DISCUSSION OF INITIAL RESULTS: UFFIZI GALLERY} 
\label{sec:evalSec}

This section evaluates the effectiveness of the DATCloud framework in accurately modeling the VASARI system, which is specifically designed to facilitate efficient visitor flow management at the Uffizi Gallery. 
\subsection{Goal}
The evaluation assesses DATCloud’s performance in reducing Modeling Time and enhancing Flexibility in Architectural Design, focusing on its efficiency, adaptability, and usability. Stakeholder feedback further validates its practicality in real-world scenarios, such as the VASARI system at the Uffizi Gallery.
% The assessment aims to determine how well DATCloud can enhance the organization and experience of visitors within this renowned cultural institution. 

% The primary focus is on Validating the framework's ability to effectively model a multi-layered architecture encompassing the edge, fog, and cloud layers. It also demonstrates the framework's effectiveness in managing the complexities of data-intensive workflows, which include modeling real-time, short-term, and long-term processes. Finally, it evaluates how well the modeled architecture aligns with the operational goals of the VASARI system.
{\color{blue}
\subsection{Metrics and Evaluation Methodology}
To evaluate DATCloud’s performance as a modeling framework, we focused on two core metrics: Modeling Time and Flexibility in Architectural Design. These metrics were chosen to reflect the framework’s ability to streamline modeling tasks, adapt to evolving requirements, and improve productivity in handling complex data-intensive architectures.

\subsubsection{Modeling Time} 
 % To quantify the efficiency improvements DATCloud offers compared to manual-based approaches.
This metric measures the total time needed to complete the modeling process, including the following tasks: 
\begin{enumerate}
    \item Workflow Definition: Time spent creating the initial architecture and data flows.
    \item System Validation: Time required to review and ensure the model aligns with system requirements. 
    \item Model Refinement: Time taken to iteratively improve and finalize the model.
\end{enumerate}

A time-tracking tool like Kimai \cite{kimai} was used to measure the time spent on each task. Each participant (e.g., architects or engineers) logged the time spent on these tasks for both manual-based methods and DATCloud. 

Time for each task was logged during the Uffizi Gallery case study using both manual methods and DATCloud.
            

\[
\text{Time Savings (\%)} = \frac{T_{\text{base}} - T_{\text{DAT}}}{T_{\text{base}}} \times 100
\]
% \noindent
      
\begin{itemize}
    \item $T_{\text{base}}$ is "Baseline Time."
    \item $T_{\text{DAT}}$ is "DATCloud Time."
\end{itemize}

% \[
% \text{Time Savings (\%)} = \frac{T_{\text{base}} - T_{\text{DAT}}}{T_{\text{base}}} \times 100

% T_{\text{base}} is  "Baseline Time."
% T_{\text{DAT}} is "DATCloud Time."
% \]


    
% \centering
% \[
% \text{Time Savings (\%)} = \frac{\text{Baseline Time} - \text{DATCloud Time}}{\text{Baseline Time}} \times 100
% \]

\subsubsection{Flexibility in Architectural Design} This metric evaluates the framework’s ability to Scale with increasing architectural complexity (e.g., adding new layers and components). Adapt to modifications or iterative changes (e.g., updating workflows or replacing components). Reuse templates or pre-defined models to simplify repetitive tasks.
Three sub-criteria were assessed, Time and steps required to add new architectural layers (e.g., fog or edge layers) or components (e.g., IoT devices or data processing nodes). Effort to update workflows or replace existing components, ensuring dependencies remain intact. Effort saved by using pre-defined templates or constructs versus creating elements from scratch. For each task, time and feedback were recorded and compared to manual-based methods.

\[
\text{Flexibility Improvement (\%)} = \frac{E_{\text{base}} - E_{\text{DAT}}}{E_{\text{base}}} \times 100
\]

\begin{itemize}
    \item $E_{\text{base}}$ is "Baseline Effort."
    \item $E_{\text{DAT}}$ is "DATCloud Effort."
\end{itemize}

\subsection{Methodology for Collecting Feedback}
Feedback was gathered from stakeholders who directly interacted with the framework during the VASARI case study at the Uffizi Gallery to evaluate DATCloud’s usability and adaptability. Participants received structured training, including an overview session, and a hands-on workshop to ensure familiarity with DATCloud's features and enable fair evaluation. Feedback was collected from stakeholders, including system architects, museum staff responsible for operational workflows, and data analysts managing IoT sensor data.

% \subsubsection{Methodology}
Stakeholders participated in one-on-one interviews lasting 30–60 minutes (Semi-Structured Interviews). A flexible interview guide ensured consistency while allowing in-depth exploration of individual experiences.  During modeling tasks, stakeholders’ interactions with DATCloud were observed to identify usability challenges and time spent on key activities.

Stakeholder feedback has refined DATCloud, improving visualization tools, streamlining templates, and enhancing validation processes. Plans are underway to expand its capabilities for specific fields like healthcare and smart cities, ensuring it remains user-friendly and adaptable.

\subsection{Results}

% The results assess DATCloud’s effectiveness with the VASARI system, highlighting time savings in modeling and increased flexibility in architectural design. The framework streamlines workflows, adapts to changing requirements, and supports scalable, multi-layered architectures. Real-world scenarios and stakeholder feedback further validate its usability and relevance across various domains.

The evaluation demonstrates that DATCloud significantly improves time savings and flexibility compared to manual-based methods.

\begin{table}[h]
\centering
\caption{Time Savings Achieved Using DATCloud}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Task}              & \textbf{$T_{\text{base}}$ (hrs)} & \textbf{$T_{\text{DAT}}$ (hrs)} & \textbf{$T_{\text{Saving}}$ (\%)} \\ \hline
Workflow Definition        & 40                          & 20                           & 50\%                       \\ \hline
System Validation          & 30                          & 20                           & 33\%                       \\ \hline
Model Refinement           & 30                          & 20                           & 33\%                       \\ \hline
\textbf{Total}             & \textbf{100}                & \textbf{60}                  & \textbf{40\%}              \\ \hline
\end{tabular}%
}
\label{tab:time}
\end{table}

Table \ref{tab:time} shows DATCloud reduces total modeling time by 40\%, with the most significant reduction observed in workflow definition (50\%) due to its use of pre-defined templates and automated tools. System validation and model refinement times were each reduced by 33\%, benefiting from automated consistency checks and reusable model structures.

\begin{table}[ht]
\centering
\caption{Flexibility Improvement Achieved Using DATCloud}
\begin{tabular}{|l|c|c|c|}
\hline
\textbf{Task}               &
\textbf{$E_{\text{base}}$ (hrs)} & \textbf{$E_{\text{DAT}}$ (hrs)} & \textbf{$T_{\text{Improvement}}$ (\%)} \\ \hline
Add Fog Layer               & 15                     & 8                      & 47\%                          \\ \hline
Add Edge Layer              & 20                     & 12                     & 40\%                          \\ \hline
Modify Workflow             & 12                     & 7                      & 42\%                          \\ \hline
Reuse Templates             & Not Applicable         & 5                      & Significant                   \\ \hline
\textbf{Total}              & 47                     & 32                     & 32\%                          \\ \hline
\end{tabular}
\label{table:flex}
\end{table}

Table \ref{table:flex} flexibility, DATCloud improved overall adaptability by 32\%, particularly in adding new layers to the architecture. Adding the fog layer was 47\% faster, and the edge layer took 40\% less time, thanks to its modular design. Workflow modifications were 42\% faster, and the use of templates for repetitive tasks provided additional, unquantifiable efficiency gains.

These results highlight DATCloud’s ability to streamline the modeling process while supporting iterative and scalable architectural designs, making it highly effective for complex, evolving systems.
}

% \subsection{Limitations}
% DATCloud has proven to offer considerable advantages, such as significantly shortening the time required for modeling tasks, enhancing the modularity of its components, and improving scalability for larger projects. Nevertheless, users faced several challenges during its implementation. Notably, the current version is missing advanced simulation capabilities that would comprehensively evaluate energy consumption and data traffic. This shortcoming restricts its effectiveness in accurately predicting resource optimization under real-world conditions, where these factors play a critical role in decision-making and efficiency.

==> acknowledgment.tex <==
\section{Acknowledgment}
The authors would like to thank Prof. Giovanni Stilo, Prof. Annabelle Gillet (Lambda+), Prof. Karthik Vaidhyanathan. And we would like to thanks Mostafa Shaer, Itay, and Roi from HP Team, Mustafa Tamim and Anas Eid from Harri Team, and , Mudassir Malik, Apurvanand Sahay, and Arsene Indamutsa as a researchers for their contributions in the evaluation.

==> application.tex <==
\section{Case Study: Uffizi Gallery}
\label{sec:casestudy}

\begin{center}
 \begin{figure*}[!h]
	\centering
	\makebox[\textwidth]
	{   	\includegraphics[width=0.90\paperwidth]{figures/test.png}
	}
	\caption{A DATCloud Application for Uffizi}
	\label{fig:app}
    \end{figure*}
\end{center}
The VASARI system, deployed at the Uffizi Gallery for visitor flow management (Figure \ref{fig:app}), was used to validate the capabilities of DATCloud. This system required the modeling of a complex, multi-layered architecture comprising IoT sensors at the edge layer, processing nodes at the fog layer, and cloud-based analytics for real-time data analysis. Using DATCloud, the structural meta-model captured the architecture of these components and their interactions, while the behavioral meta-model defined workflows such as visitor tracking and queue management.

% DATCloud demonstrated significant improvements over traditional manual modeling methods, achieving a 40\% reduction in modeling time and a 32\% improvement in flexibility. Stakeholder feedback highlighted the framework’s intuitive graphical DSLs and the ability to reuse templates, which streamlined iterative changes during the modeling process. These results validate DATCloud’s effectiveness in handling real-world, data-intensive systems and demonstrate its potential for broader applications in domains such as healthcare and smart cities.



==> background.tex <==
\section{Background}

This section provides insights about the ISO/IEC/IEEE 42010 standard and more details concerning data-intensive applications.

\subsection{IEEE/ISO/IEC 42010 Architecture Description}
\label{42010}
This paper explores the fundamental components of architecture description for Data-Intensive Applications. We rely on the ISO/IEC/IEEE 42010:2011 \cite{42010}, Systems and software engineering — Architecture description standard, to guide our investigation. The goal is to establish effective practices for documenting and analyzing software, systems, and enterprise architectures to ensure they can be comprehended, documented, analyzed, and implemented. Architecture descriptions can take various forms, from casual to highly specified models. 
% The architecture content model plays a crucial role in this process.
\subsection{Data-Intensive Applications}
Data-intensive applications are advanced software systems that effectively handle large amounts of data. These applications are specifically designed to manage and manipulate data, primarily focusing on storing and processing significant volumes of data. Moreover, 
% they can handle various data types, such as structured, unstructured, and semi-structured \cite{dataintensive}. These applications are prized for their ability to process vast amounts of data, which can be challenging and rewarding. 
Despite the complexity of processing real-time data, data-intensive applications can provide businesses with valuable insights \cite{kleppmann2019designing}.
Many companies have realized the advantages of data-intensive development and are now actively implementing it. This approach necessitates \textit{ collecting, storing, and processing vast amounts of data}, making it an essential aspect of their operations.

\subsection{Cloud-Fog-Edge Architecture}
The cloud-fog-edge architecture is a comprehensive layered computing model designed to optimize data processing efficiency and scalability across distributed networks. In this architecture, data processing tasks are effectively allocated among three layers: the cloud, fog, and edge. The cloud layer is responsible for managing high-complexity, large-scale data processing, and storage, making it suitable for handling significant volumes of data. The fog layer acts as an intermediary, enabling real-time data processing closer to end-users, which improves responsiveness. Meanwhile, the edge layer focuses on processing data directly at the source, significantly reducing latency.

This multi-layered approach is especially beneficial for data-intensive applications, as it facilitates a seamless flow of information across various devices and systems. It supports diverse data views and enhances real-time decision-making, leveraging the strengths of each layer to cater to specific processing needs.
